Randomized Truthful Auctions with Learning Agents

We study a setting where agents use no-regret learning algorithms to participate in repeated auctions. \citet{kolumbus2022auctions} showed, rather surprisingly, that when bidders participate in second-price auctions using no-regret bidding algorithms, no matter how large the number of interactions $T$ is, the runner-up bidder may not converge to bidding truthfully. Our first result shows that this holds for \emph{general deterministic} truthful auctions. We also show that the ratio of the learning rates of the bidders can \emph{qualitatively} affect the convergence of the bidders. Next, we consider the problem of revenue maximization in this environment. In the setting with fully rational bidders, \citet{myerson1981optimal} showed that revenue can be maximized by using a second-price auction with reserves.We show that, in stark contrast, in our setting with learning bidders, \emph{randomized} auctions can have strictly better revenue guarantees than second-price auctions with reserves, when $T$ is large enough. Finally, we study revenue maximization in the non-asymptotic regime. We define a notion of {\em auctioneer regret} comparing the revenue generated to the revenue of a second price auction with truthful bids. When the auctioneer has to use the same auction throughout the interaction, we show an (almost) tight regret bound of $\smash{\widetilde \Theta(T^{3/4})}.$ If the auctioneer can change auctions during the interaction, but in a way that is oblivious to the bids, we show an (almost) tight bound of $\smash{\widetilde \Theta(\sqrt{T})}.$

==> always-alloc.tex <==
\section{Optimal Randomized Auction that Always Allocates}\label{sec:optimal auction for fixed valuations}
If the valuations $v_H, v_L$ are known, what is the optimal randomized
allocation rule that always allocates the item? The motivation
is that in the setting where the auctioneer can change the randomness
parameter of the auction during the interaction, it can first
start with some ``aggressive'' randomization that will drive 
the convergence of the bidders to truthful bidding. Then, the auctioneer
can essentially infer the valuation of the bidders and then switch
to the optimal auction in the remaining rounds. The first observation
is that if the allocation rule is not symmetric, then the auctioneer
can easily extract all the welfare. This is formalized
in the following claim.
\begin{claim}[Optimal Asymmetric Auction]\label{clm:asymmetric optimal auction when valuations are known}
    Assume that the auctioneer has access to $v_H, v_L$.
    Then, for any $\varepsilon > 0$, 
    there is an auction that allows the auctioneer to 
    generate revenue $\rev = v_H - \varepsilon.$
\end{claim}
\begin{proof}
    Let $\alpha = \frac{v_H - \varepsilon}{v_L}.$ Consider
    the following auction. The auctioneer first inflates the
    bid of the low bidder by $\alpha$ and then runs a second
    price auction between the bid of the high agent
    and the inflated bid of the low agent. It is not
    hard to see that the allocation rule is monotone,
    hence the auction is truthful, hence
    truthful bidding is a (weakly) dominant strategy. 
    We can see that under truthful bidding the high
    type always wins the auction and pays
    $v_H - \varepsilon.$
\end{proof}


The auction that gives rise to the previous result is not
very satisfactory, since it discriminates between the two
agents and puts the high bidder at some disadvantage. Hence,
a natural question is whether there is some inherent obstacle
to full welfare extraction under symmetric auctions\footnote{Formally,
an auction is symmetric if $x_H(b,b') = x_L(b',b), \forall b,b' \in [0,1]$, where $x_H(\cdot,\cdot), x_L(\cdot,\cdot)$, are the allocation
probabilities of the high, low player, respectively.}.
The next result shows that, indeed, symmetric auctions that always
allocate the item can extract at most $\rev = (v_L + v_H)/2.$

\begin{theorem}[Optimal Symmetric Auction]\label{thm:symmetric optimal auction when valuations are known}
    Assume that the auctioneer has access to $v_H, v_L$. Then, the
    revenue optimal symmetric auction that always allocates the item
    extracts revenue $\rev = (v_H + v_L)/2.$ Let $x_H(b_H,b_L), x_L(b_H,b_L)$ be the allocation probabilities of the high, low
    type, respectively, under bid profile $(b_H,b_L).$ Then, such an auction
    is optimal if and only if it satisfies:
    \begin{enumerate}
        \item $x_H(v_H,v_L) = 1.$
        \item $x_L(b_H,v_L) = 1, \forall b_H \in [0,v_L).$
        \item $x_L(b_H,v_L) = x_H(b_H,v_L) = 1/2,
        \forall b_H \in [v_L, v_H).$
    \end{enumerate}
\end{theorem}
\begin{proof}
Let us start by writing the revenue maximization problem. Using
Myerson's payment formula, it suffices to specify the allocation
rule. Since we restrict our attention to monotone allocation rules,
we have that
\begin{align}\label{eq:optimal single shot auction for known vals}
    \sup_{x_L(\cdot,\cdot), x_H(\cdot,\cdot)}& \left\{v_H\cdot x_H(v_H, v_L) - \int_{0}^{v_H} x_H(z,v_L) dz + v_L\cdot x_L(v_H, v_L) - \int_{0}^{v_L} x_L(v_H, z) dz\right\} \\
    \text{ s.t. } & x_H(b_H, b_L) + x_L(b_H,b_L) = 1, \forall b_L, b_H \in [0,1] & \text{(item is always allocated)} \nonumber\\
    & x_H(b_H, b_L) = x_L(b_L,b_H), \forall b_L, b_H \in [0,1] & \text{(symmetry condition)} \nonumber \\
    & x_H(\cdot, b_L) \text{ non-decreasing }, \forall b_L \in [0,1] \nonumber\\
    & x_L(b_H, b_L) \text{ non-decreasing }, \forall b_H \in [0,1] \nonumber
\end{align}
We start by simplifying the above optimization problem. The condition
$x_H(b_H,b_L) + x_L(b_H,b_L) = 1$ allows us to use a single function
$x(\cdot,\cdot) \coloneqq x_H(\cdot,\cdot)$ in order to express
the allocation probabilities. Under the new notation, the symmetry
condition of \Cref{eq:optimal single shot auction for known vals}
is equivalent to $x(b_H, b_L) = 1 -x(b_L, b_H).$
Moreover, the monotonicity conditions imply that $x(\cdot,b_L)$
is non-decreasing, for all $b_L \in [0,1]$, and $x(b_H,\cdot)$ is
non-increasing for all $b_H \in [0,1].$
Then, we can rewrite \Cref{eq:optimal single shot auction for known vals} as
\begin{align}\label{eq:simplified optimal single shot auction for known vals}
    \sup_{x(\cdot,\cdot)}& \left\{v_H \cdot x(v_H, v_L) - \int_{0}^{v_H} x(z,v_L) dz
    + v_L\cdot (1-x(v_H, v_L)) - \int_{0}^{v_L}(1-x(v_H, z))dz \right\}\\
    \text{ s.t. }& x(b_H,b_L) = 1 - x(b_L,b_H), \forall b_H,b_L \in [0,1] &\text{ (symmetry condition) }\nonumber \\
                & x(b_H,\cdot) \text{ non-increasing}, \forall b_H \in [0,1] \ \nonumber \\
                & x(\cdot, b_L) \text{ non-decreasing}, \forall b_L \in [0,1]  \nonumber 
\end{align}
Let us denote by $R$ the set of feasible allocations, i.e., the ones 
that satisfy the constraints of \Cref{eq:simplified optimal single shot auction for known vals}.
Then, we can write the problem as follows:
\begin{align*}
     \sup_{x(\cdot,\cdot) \in R} \left\{v_H \cdot x(v_H, v_L) - \int_{0}^{v_H} x(z,v_L) dz
    + v_L\cdot (1-x(v_H, v_L)) - \int_{0}^{v_L}\left(1-x(v_H, z)\right)dz \right\} &\stackrel{\text{symmetry condition}}{=}\\ 
    v_L + \sup_{x(\cdot,\cdot) \in R} \left\{(v_H - v_L) \cdot x(v_H, v_L) - \int_{0}^{v_H} x(z,v_L) dz
   - \int_{0}^{v_L}x(z,v_H)dz \right\} &= \\
   v_H - \inf_{x(\cdot,\cdot) \in R, x(v_H, v_L) = 1} \left\{\int_{0}^{v_L}(x(z,v_H) + x(z,v_L))dz + \int_{v_L}^{v_H} x(z,v_L) dz   \right\} \,,
\end{align*}
where the last step follows by observing that
$x(v_H,v_L)$ can make the allocation rule feasible
and it does not affect the remaining of the optimization problem.
Observe that the symmetry condition implies that $x(v_L,v_L) = 1/2$,
and due to the monotonicity condition we have that
$\int_{v_L}^{v_H} x(z,v_L) dz \geq 1/2\cdot (v_H - v_L).$
Since $x(z,v_L), x(z,v_H) \geq 0$, 
the revenue the auctioneer can extract is at most
$v_H - (v_H - v_L)/2 \leq (v_H - v_L)/2.$ 
Notice that the equality is achieved if and only if
$\int_{0}^{v_L} (x(z,v_H) + x(z,v_L))dz = 0$ and
$x(z,v_L) = 1/2, \forall z \in [v_L,v_H).$
Notice that the first condition, due to monotonicity,
is equivalent to $x(z,v_L) = 0, \forall z \in [0, v_L).$
Let $R' = R \cap \left\{x(v_H, v_L) = 1\right\}\cap \left\{x(z,v_L) = 0, \forall z < v_L \right\} \cap \left\{ x(z,v_L) = 1/2, \forall z \in [v_L,v_H) \right\}$. Notice
that all $x(\cdot,\cdot) \in R'$ satisfy $x(v_L,v_L) = 1/2$.
Then,
\begin{align*}
    v_H - \inf_{x(\cdot,\cdot) \in R, x(v_H, v_L) = 1} \left\{\int_{0}^{v_L}(x(z,v_H) + x(z,v_L))dz + \int_{v_L}^{v_H} x(z,v_L) dz   \right\} &=
    v_H - \inf_{x(\cdot,\cdot) \in R'} \left\{\int_{v_L}^{v_H} x(z,v_L) dz   \right\} \\
    &=
    v_H - (v_H - v_L)/2  \\
    & = \frac{v_L + v_H}{2} \,.
\end{align*}
To sum up, the auction works as follows:
\begin{itemize}
    \item If one bid is strictly less than $v_L$ and the other bid is at least $v_L$, it allocates to the bidder with $v_L$.
    \item If both bids are in $[v_L, v_H)$ it allocates randomly
    between the two.
    \item If one bid is at least $v_H$ and the other bid is strictly less
    than $v_H$ then it allocates to the bidder with $v_H.$
\end{itemize}
Observe that there are more than one auctions that satisfy
these conditions.
\end{proof}


==> further-related-work-apx.tex <==
\section{Further Related Work}\label{apx:further-related-work}

==> intro.tex <==
\section{Introduction}\label{sec:intro}
The use of learning algorithms to bid in repeated auctions, especially
in the setting of online advertising, has increased significantly
in the past few years. Many companies provide
such automated tools that bid on behalf of advertisers
who are trying to optimize their campaigns
\citep{googleAutoBidding}. Classical auction
design has focused on analyzing scenarios
where the participating agents are \emph{fully rational},
which means that they are able to bid in a way
that maximizes their utility. Hence, it is natural
to ask whether such bidding algorithms exhibit
the same qualitative behavior that the classical
theory predicts. Recently, a surprising result
by \citet{kolumbus2022and}
showed that when two agents that have valuations $v_L, v_H$
for some item
participate in repeated second-price auctions
using \emph{no-regret} learning algorithms
that bid on their behalf do not converge to bidding
truthfully. In particular, the no-regret algorithm bidding for the agent with the higher valuation converges to bidding
uniformly between $v_L, v_H$, whereas the one for the agent
with the lower valuation converges to a bidding
distribution with mean strictly less than $v_L$.
This behavior is problematic for at least two reasons.
Firstly, the revenue of the auctioneer 
is determined by the lower bid: in this case, this is strictly
less than in the fully-rational case. Secondly, if we consider the \emph{meta-game}
in which the agents determine what valuation
they should report to the bidding algorithms,
\citet{kolumbus2022auctions} show that the agent with the
lower valuation has an incentive to misreport
and submit a valuation strictly larger than $v_L$ to its bidding algorithm. In a similar spirit,
\citet{banchio2022artificial} studied a setting
where two agents participate in repeated \emph{first-price}
auctions using \emph{$Q$-learning} algorithms. They show
that these algorithms exhibit collusive behavior
and the revenue that is generated is significantly lower
than what the theory predicts. These two findings
motivate the main question we study in our work:
\emph{Can we design auctions in which no-regret
learning agents converge to bidding truthfully and have
good revenue guarantees for the auctioneer?}

Our first result, which builds upon and extends the work of 
\citet{kolumbus2022auctions}, shows that this goal is not achievable 
if we restrict ourselves to deterministic auctions. 
Specifically, we show that in any deterministic
auction, the agent with lower valuation
converges to bidding strictly below its true value.
Given this negative result for deterministic auctions, we focus on \emph{randomized} auctions. For such auctions, we provide
a black-box transformation from any auction $A$ to 
an auction $A'$ that has the following two properties:
i) no-regret learning algorithms
that participate in $A'$ converge
to bidding truthfully, 
ii) the pointwise difference in the allocation and the payment
between auctions $A$ and $A'$ is negligible \anupamnote{Should we say "as $T \to \infty$" right here?}. 
\ganote{Just to make sure I understand -- the claim is that for any input bid vector, the difference in allocation and payment is small. However, for any time period, the difference could be large. In particular, as time goes by, we expect the difference in allocation and payment between the two mechanisms to increase, right?}
As a corollary of this result we can show that the revenue-maximizing auction in this setting is randomized, which is in stark contrast with the seminal result
of \citet{myerson1981optimal} who showed that the revenue 
optimal auction when the agents are rational is deterministic. As another application of this result,
we can show how to create ``meta-games''
where, as $T \rightarrow \infty$,
each agent has only a negligible advantage of
misreporting its value to the bidding algorithm.

Next, we consider the non-asymptotic regime
and we design auctions that induce truthful bidding
from no-regret learning algorithms
and have strong revenue guarantees. We mainly
focus our attention on the \emph{prior-free}
setting where the auctioneer does not have 
any distributional knowledge about the
valuation of the bidders. In order
to measure the performance of the auctions we compare
the total expected revenue generated across
$T$ rounds of interaction with the revenue that would
be generated by the second price auction
if the bidders were bidding truthfully. \grigorisnote{Do we need 
to add further motivation about this benchmark?}\anupamnote{I would say yes.} We call the \alert{difference between these two quantities}
the \emph{modified regret}. Firstly,
we show that if the designer uses the same auction across 
all $T$ rounds and is restricted to choosing
an auction from a natural and expressive class of auctions, then it cannot achieve
modified regret that is better than $\widetilde{O}(T^{3/4}).$
(Roughly speaking, this class $\calA$
consists of auctions that are convex combinations of auctions
whose description does not depend on $T$, even though---importantly--- the multipliers of these convex combination are allowed to depend
on $T.$)
Then, we show that if the designer is allowed to change the auction once, but, crucially, in a way that does not depend
on the bid history, then it can achieve modified regret
$\widetilde{O}(\sqrt{T}).$ We prove that this 
bound on the modified regret is optimal, even \alert{in the Bayesian setting where} the auctioneer has distributional knowledge about the valuations of the bidders. As 
a byproduct of our result, we identify
an auction that leads to the fastest convergence to 
truthful bidding from no-regret learning agents.

\subsection{Related Work}\label{sec:related-work}
The pioneering work of \citet{hart2000simple} showed that when players
deploy no-regret algorithms to participate in games
they converge to \emph{coarse-correlated equilibria}.
Recently, there has been a growing interest in the study
of no-regret learning in repeated auctions. The empirical
study of \citet{nekipelov2015econometrics} showed that the bidding
behavior of advertisers on Bing is consistent
with the use of no-regret learning algorithms that bid 
on their behalf. Subsequently, \citet{braverman2018selling}
showed, among other things, that when a seller faces a no-regret buyer
in repeated auctions it can extract the whole welfare
as its revenue. A very recent work \citep{cai2023selling} extended
some of the previous results to the setting with multiple
agents. 

The most closely related works to our setting
are \citet{feng2021convergence, deng2021firstPrice, kolumbus2022auctions, banchio2022artificial,rawat2023designing}. All these works
study the long-term behavior of bidding algorithms that participate in 
repeated auctions, focusing on first-price and second-price auctions,
but they give qualitatively different results. This is because they
make different assumptions across two important axes: the type of
learning algorithms that the bidders use and whether their 
valuation is \emph{persistent} across the interaction
or it is freshly drawn in each round. \citet{feng2021convergence}
studied the convergence of no-regret learning algorithms
that bid repeatedly in second-price and first-price auctions, where
all agents have i.i.d. valuation that are redrawn in every round
from a discrete distribution that has non-negligible mass on each point.
They show that in this setting the bidders exhibit the same-long
term behavior in both second-price and first-price auctions that 
classical theory predicts, i.e., the bids in second-price auctions
are truthful and the bids in first-price auctions form
Bayes-Nash equilibria. 

\citet{kolumbus2022auctions} studied the
same setting with a subtle, but crucial, difference: the valuations
of the agents are persistent across the execution and they
are not resampled from some distribution at every iteration.
Interestingly, they showed that in the case of two bidders with
in second-price
auctions, the agent that has the highest valuation will end up
bidding uniformly between the low valuation and its valuation,
whereas the agent with the low type will end up bidding 
strictly below its valuation. Intuitively, in their setting
the high type bidder quickly learns to bid
above the valuation of the low type bidder and always win the auction,
and thus the low type does not get enough signal to push its bid distribution
up to its valuation. On the other hand, when the valuations are redrawn
as in \citet{feng2021convergence}, the competition that the agents face varies.
In the long run, this gives enough information to the algorithms
to realize that bidding truthfully is the optimal strategy. In the 
case of first-price auctions where the agents have
persistent valuations \anupamnote{Similar to what?}\grigorisnote{I rephrased it, does it make more sense now?}
both \citet{kolumbus2022auctions, deng2021firstPrice} provide
convergence guarantees of no-regret learning algorithms.

\citet{banchio2022artificial,rawat2023designing} diverge from the previous works
and consider agents that use $Q$-learning algorithms instead
of no-regret learning algorithms. Their experimental findings show that
in first-price auctions, such algorithmic bidders exhibit
collusive phenomena, whereas  they converge
to truthful bidding in second-price auctions. One of the main reasons for these
phenomena is the \emph{asynchronous} update used by the $Q$-learning
algorithm. The collusive behavior of such algorithms 
has also been exhibited in other settings
\citep{calvano2020protecting,asker2021artificial,asker2022artificial,den2022artificial,epivent2022algorithmic,asker2022impact}.
Notably, \citet{bertrand2023qlearners} formally proved that $Q$-learners
do indeed collude when deployed in repeated prisoner's dilemma games.

In a related line of work, \citet{zhang2023steering}
study the problem of steering no-regret learning agents to 
some particular equilibrium. They show that the auctioneer can use 
\emph{payments} in order to incentivize the algorithms to converge
to a particular equilibrium that the designer wants them to.
\grigorisnote{TODO: mention something more about the setting they consider.}
One way to interpret our results is that \emph{randomization}
is a way to achieve some kind of equilibrium steering in repeated auctions.
\grigorisnote{Any other works we should cite?}

Diverging slightly from the setting we are
considering in our work, some recent papers
have illustrated different advantages of
using randomized auctions instead
of deterministic ones. In particular, \citet{mehta2022auction, liaw2023efficiency}
showed that there are randomized auctions which induce equilibria
with better welfare guarantees for value-maximizing
autobidding agents compared to deterministic ones.
In the setting of revenue maximization in the presence
of heterogeneous rational buyers, \citet{guruganesh2022prior} showed that randomization
helps when designing prior-free auctions with
strong revenue guarantees, when the valuations
of the buyers are drawn
independently from, potentially, non-identical distributions.










% \grigorisnote{TODO: comment on the differences between \cite{feng2021convergence, kolumbus2022auctions, banchio2022artificial}
% and why they get the seemingly conflicting results. This 
% paper is very recent \cite{rawat2023designing} and is also relevant. It's
% mostly experimental but the take-away is that auctioneers should
% be using second price auctions when the agents are no-regret
% learners to avoid the collusion phenomena of first price auctions.
% They consider a similar setting as \cite{banchio2022artificial}
% and, importantly, the valuations of all the bidders are the
% same (as in \cite{banchio2022artificial}. This is basically the only
% setting where second price auction leads to truthful bidding
% under no-regret learning and this is something we should
% highlight in our work (it is also supported by the 
% experiments in \cite{banchio2022artificial} where they consider
% bidders with different valuations.) Another important
% paper to discuss is \cite{deng2021firstPrice} which shows that
% learning agents who participate in first price auctions
% converge to the correct Nash equilibrium (in contrast with 
% the empirical RL works). The catch is that in \cite{deng2021firstPrice}
% the learners are using the \emph{correct} algorithms
% and do not suffer from the asynchronicity issue of \cite{banchio2022artificial, rawat2023designing}.
% \cite{asker2022artificial} is also relevant (and references therein).\cite{den2022artificial} doubt the collusion arguments. Other econ papers \cite{asker2021artificial,asker2022artificial}
% also claim that 
% synchronous learning leads to competitive 
% pricing and this behavior in general 
% is heavily dependent on the learning algorithm.
% To the best of our knowledge, this is 
% the first paper that studied
% collusive learning outcomes in markets
% \cite{calvano2020protecting}. The argument
% that this is mostly an issue with $Q$-learning
% is also made by \cite{den2022artificial} (Section 5). They
% also show that $Q$-learning loses against Exp3.
% This paper also questions the collusion 
% results \cite{epivent2022algorithmic}. This paper
% \cite{asker2022impact} supports the claim that collusion
% happens when there is bandit feedback under $Q$-learning
% but when there is full feedback there is no collusion.
% Very recently, \cite{bertrand2023qlearners} proved
% that $Q$-learners collude when deployed in repeated
% prisoner's dilemma games.

% Tangentially related work, same objective but 
% different types of games, \cite{zhang2023steering}.

% We also need to discuss \cite{braverman2018selling, cai2023selling}. They consider the problem
% of maximizing revenue in repeated auctions
% while selling to (multiple) no-regret learners.
% Importantly, the bidders draw a fresh valuation
% in each round.
% They present a very complicated and unnatural auction
% that extracts the full welfare when the bidders
% are not constrained to never overbid. They show that
% there is a ``smart'' no-regret learning algorithm
% that cannot be exploited so the auctioneer
% always gets Myerson's revenue. Finally, they consider
% ``simpler'' no-regret learning algorithms that are
% constrained to never overbid. When they are is a
% single buyer, they characterize the optimal
% revenue, which is strictly greater than Myerson's
% revenue and strictly worse than the full welfare. 
% For multiple bidders such a characterization remains
% elusive and \cite{cai2023selling} identify
% various difficulties in extending it to this setting.

% \cite{golrezaei2017boosted} consider boosted second 
% price auctions where the bid of each person is boosted
% by some factor. They show that this approach is more robust
% and leads to better revenue than using a personalized
% reserve price. This is mostly empirical I think and 
% has a similar spirit to \cite{guruganesh2022prior}.

% \cite{anunrojwong2023robust} consider robust prior-free
% mechanisms with side information, which
% is of the form of a lower bound and an upper bound
% on the support of the valuation. They propose a pooling
% mechanism that is parametrized by a threshold $\tau$ and
% works as follows: if the highest bid
% is above $\tau$ then they allocate to this bidder,
% otherwise they allocate uniformly at random. This is 
% similar to the mechanism we propose
% in \Cref{sec:optimal auction for fixed valuations}. 

% \cite{deng2019prior} this paper is also worth mentioning.
% It is a similar setting as \cite{braverman2018selling}
% but now instead of having i.i.d. valuations for the 
% buyer, they are chosen adversarially and possibly 
% adaptively. A special case is our setting where we consider
% one learning agent
% and one that is always truthful. Importantly, their
% mechanisms are fixed at all times.

% \cite{diakonikolas2012efficiency} this paper shows that randomized
% auctions that achieve any point in the Pareto frontier of revenue-efficiency
% can be computed in polynomial time whereas deterministic ones cannot.
% }

% \subsection{Comments on Prior Results}\label{sec:comments on prior results}
%     We need to have a detailed comparison with \cite{feng2021convergence, kolumbus2022auctions, banchio2022artificial}. These works study what happens
%     when learning agents participate in repeated auctions and
%     they focus on first-price auctions and second-price
%     auctions. 
%     We can compare them across these axes:
%     \begin{itemize}
%         \item Persistence of valuations: \cite{kolumbus2022auctions, banchio2022artificial} 
%         use persistent valuations, whereas \cite{feng2021convergence} draw fresh valuations
%         after each round. Importantly, they make
%         the assumption that the supports are the same
%         and all the distributions put at least $\tau$ 
%         mass on every point of the support. Moreover,
%         \cite{banchio2022artificial} mostly focus on
%         $v_L = v_H.$
%         \item Learning algorithms: \cite{feng2021convergence, kolumbus2022auctions}
%         use no-regret learning algorithms whereas
%         \cite{banchio2022artificial} use $Q$-learning.
%         \item Results:
%         \begin{itemize}
%             \item Second price auctions: \cite{kolumbus2022auctions} show that
%             no-regret learning in second-price auctions
%             does not always converge to truthful bidding, 
%             whereas \cite{feng2021convergence, banchio2022artificial} show that it does. 
%             The reason is that \cite{feng2021convergence}
%             use non-persistent valuations and the
%             distributions are ``fat'', and \cite{banchio2022artificial} use $v_H = v_L.$
%             \item First price auctions: \cite{feng2021convergence, kolumbus2022auctions}
%             show convergence to truthful bidding whereas
%             \cite{banchio2022artificial} show collusion.
%             This is because of the asynchronous update
%             rule of $Q$-learning.
%         \end{itemize}
        
%     \end{itemize}
    
    


% \subsection{Preliminaries}\label{sec:prelim}
% \andresnote{What is the point of this section? shouldn't this be exactly the model section?}
% \grigorisnote{Sure, we can just have a "model" section where we introduce whatever preliminaries are necessary.}
% \paragraph{Mechanism Design.}

% \paragraph{No-Regret Learning.}

% \paragraph{Notation.}

==> olddefs.tex <==
\usepackage[utf8]{inputenc}
\oddsidemargin=-0.1in 
\evensidemargin=-0.1in 
\topmargin=-.5in
\textheight=9in 
\textwidth=6.5in
\parindent=18pt

\bibliographystyle{alpha}

\usepackage{mdframed}
\usepackage{algorithm,algorithm,multicol}
\usepackage{pgfplots}


% \usepackage[usenames,dvipsnames]{xcolor}
\definecolor{Gred}{RGB}{219, 50, 54}
\definecolor{Ggreen}{RGB}{60, 186, 84}
\definecolor{Gblue}{RGB}{72, 133, 237}
\definecolor{Gyellow}{RGB}{247, 178, 16}
\definecolor{ToCgreen}{RGB}{0, 128, 0}
\definecolor{myGold}{RGB}{231,141,20}
\definecolor{myBlue}{rgb}{0.19,0.41,.65}
\definecolor{myPurple}{RGB}{175,0,124}
\definecolor{niceRed}{RGB}{153,0,0}
\definecolor{niceRed}{RGB}{190,38,38}
\definecolor{blueGrotto}{HTML}{059DC0}
\definecolor{royalBlue}{HTML}{057DCD}
\definecolor{navyBlueP}{HTML}{0B579C}
\definecolor{limeGreen}{HTML}{81B622}
\definecolor{nicePink}{RGB}{247,83,148}

\usepackage{cmap}
\usepackage[T1]{fontenc}
\usepackage{bm}
\pagestyle{plain}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{breqn}


\allowdisplaybreaks

\usepackage{graphicx, ucs}

\usepackage{subcaption}
\usepackage{rotating}
\usepackage{float}
\usepackage{tikz}

\usepackage{algorithm, caption}
\usepackage[noend]{algpseudocode}
\usepackage{listings}

\usepackage{enumitem}


\usepackage[pagebackref]{hyperref}
\hypersetup{
	colorlinks = true,
	urlcolor = {myPurple},
	linkcolor = {royalBlue},
	citecolor = {nicePink}
}
\usepackage[nameinlink]{cleveref}


\usepackage{multirow}
\usepackage{array}

\usepackage{chngcntr}

\counterwithin*{equation}{section}
\usepackage{chngcntr}
\usepackage{soul}
%\usepackage{dsfont}
\usepackage{nicefrac}

\usepackage{fancyhdr}
\fancyhf{}
\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}
\fancyheadoffset{0pt}
\cfoot{\thepage}


\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter

\newenvironment{Enumerate}
{\def\usecounter{\compactify\latexusecounter}
	\begin{enumerate}}
	{\end{enumerate}\let\usecounter=\latexusecounter}

\newenvironment{Itemize}{\begin{itemize}\setlength{\itemsep}{0pt}\setlength{\topsep}{0pt}\setlength{\partopsep}{0 in}\setlength{\parskip}{0 pt}}{\end{itemize}}

\definecolor{myC}{rgb}{0, 255, 255}
\definecolor{myY}{rgb}{204, 204, 0}
\definecolor{myM}{rgb}{255, 0, 255}
\definecolor{secinhead}{RGB}{249,196,95}
\definecolor{lgray}{gray}{0.8}



\usepackage{svg}

% Defs

\newtheorem{theorem}{Theorem} 
\newtheorem*{theorem*}{Theorem} 
\newtheorem*{proposition*}{Proposition} 
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{openquestion}{Open Question}
\newtheorem{answer}{Answer}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{inftheorem}{Informal Theorem}

\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{observation}{Observation}
\newtheorem{example}{Example}
\newtheorem{examples}[theorem]{Example}

% probability and other mathops
\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\E}{\mathop{\bf E\/}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\Var}{\mathop{\bf Var\/}}
\newcommand{\Cov}{\mathop{\bf Cov\/}}
\newcommand{\er}{\mathrm{er}}
\newcommand{\bin}{\mathrm{bin}}
\newcommand{\SP}{\mathrm{SP}}
\newcommand{\vars}{\mathrm{Var}}

% terms
\newcommand{\poly}{\textnormal{poly}}
\newcommand{\polylog}{\textnormal{polylog}}
\newcommand{\size}{\textnormal{size}}
\newcommand{\sgn}{\textnormal{sgn}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\supp}{\textnormal{supp}}
\newcommand{\oig}{\mathrm{OIG}}
\newcommand{\medboost}{\mathrm{MedBoost}}
\newcommand{\fat}{\mathrm{fat}}
\newcommand{\med}{\mathrm{Median}}
\newcommand{\onlinedim}{\mathbb D^{\mathrm{onl}}}
\newcommand{\rtruth}{\mathrm{rTruth}}
\newcommand{\spr}{\mathrm{SP}}
\newcommand{\rev}{\mathrm{Rev}}
\newcommand{\softmax}{\mathrm{SoftMax}}
\newcommand{\reg}{\mathrm{Reg}}


% number systems
\newcommand{\reals}{\mathbb R}
\newcommand{\complex}{\mathbb C}
\newcommand{\nats}{\mathbb N}
\newcommand{\natszero}{\mathbb N_0}
\newcommand{\natsinf}{\mathbb N_{\infty}}
\newcommand{\ints}{\mathbb Z}
\newcommand{\rats}{\mathbb Q}

\newcommand{\eps}{\epsilon}

% calligraphic letters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\hI}{\mathbb{I}}
\newcommand{\hN}{\mathbb{N}}

% bold
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\ba}{\boldsymbol{a}}

% other defs
\def\l{\ell}
\def\<{\langle}
\def\>{\rangle}

% Distributions
\newcommand{\Be}{\textit{Be}}
\newcommand{\Bin}{\textit{Bin}}
\newcommand{\N}{\calN}
\newcommand{\Z}{\calZ}
\newcommand{\TG}{\calT\calG}
\newcommand{\Geo}{\textit{Geo}}

% macros
\newcommand{\lr}[1]{\mathopen{}\left(#1\right)}
\newcommand{\Lr}[1]{\mathopen{}\big(#1\big)}
\newcommand{\LR}[1]{\mathopen{}\Big(#1\Big)}

\newcommand{\lrbra}[1]{\mathopen{}\left[#1\right]}
\newcommand{\Lrbra}[1]{\mathopen{}\big[#1\big]}
\newcommand{\LRbra}[1]{\mathopen{}\Big[#1\Big]}

\newcommand{\norm}[1]{\|#1\|}
\newcommand{\lrnorm}[1]{\mathopen{}\left\|#1\right\|}
\newcommand{\Lrnorm}[1]{\mathopen{}\big\|#1\big\|}
\newcommand{\LRnorm}[1]{\mathopen{}\Big\|#1\Big\|}

\newcommand{\lrset}[1]{\mathopen{}\left\{#1\right\}}
\newcommand{\Lrset}[1]{\mathopen{}\big\{#1\big\}}
\newcommand{\LRset}[1]{\mathopen{}\Big\{#1\Big\}}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\lrabs}[1]{\mathopen{}\left|#1\right|}
\newcommand{\Lrabs}[1]{\mathopen{}\big|#1\big|}
\newcommand{\LRabs}[1]{\mathopen{}\Big|#1\Big|}



\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\def\wt{\widetilde}
\def\wh{\widehat}
\def\eps{\varepsilon}
\def\vec{\bm}

\def\dtv{\mathrm{TV}}
\def\rSTAT{\texttt{rSTAT}}
\def\err{\mathrm{er}}
\def\SPA{\mathrm{SPA}}


\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}%
\newcommand*{\QEDB}{\hfill\ensuremath{\square}}%

\newcommand{\grigorisnote}[1]{{\color{purple}{Grigoris: #1}}}
\newcommand{\andresnote}[1]{{\color{blue}{Andres: #1} }}
\newcommand{\ganote}[1]{{\color{green}{Gagan: #1} }}
\newcommand{\anupamnote}[1]{{\color{red}{Anupam: #1} }}


\newmdtheoremenv{theo}{Informal Theorem}
\newmdtheoremenv{definition-frame}{Definition}


\makeatletter
\renewenvironment{abstract}{%
	\if@twocolumn
	\section*{\abstractname}%
	\else %% <- here I've removed \small
	\begin{center}%
		{\bfseries \large\abstractname\vspace{\z@}}%  %% <- here I've added \Large
	\end{center}%
	\quotation
	\fi}
{\if@twocolumn\else\endquotation\fi}
\makeatother


==> omitted-details-deterministic.tex <==
\section{Omitted Details from \Cref{sec:deterministic auctions}}\label{apx:deterministic}



==> omitted-details-finite.tex <==
\section{Omitted Details from \Cref{sec:no-regret-learning-auctioneer}}\label{apx:finite-horizon}

==> omitted-details-randomized.tex <==
\section{Omitted Details from Section \ref{sec:randomized-truthful-auctions}}\label{apx:randomized-asymptotic}


==> one-learner.tex <==
\grigorisnote{Please ignore the next section.}
\section{Intermediate Setting: One Learner, One Truthful}
\label{sec:one learner, one truthful}
In this section we explore an intermediate setting in order 
to develop some more intuition where we have two bidders
with distinct valuations $v_L, v_H, v_L < v_H$
that repeatedly participate in an auction. Importantly,
the high valuation agent is more sophisticated and bids 
truthfully in the auction, but the low valuation
agent uses a no-regret learning algorithm to participate in
it. The timeline of the interaction works as follows:
\begin{itemize}
    \item The auctioneer commits to an auction format given
    the distribution $F$ of the valuations of the bidders.
    \item The valuations $v_L, v_H$ are drawn i.i.d. from $F.$
    \item The bidders participate in the auction, 
    the low valuation bidder uses a no-regret learning 
    algorithm while the high valuation bidder 
    is always truthful.
\end{itemize}



\subsection{Low Valuation Bidder is Truthful}\label{sec:low valuation truthful, high valuation learner}

We first consider the setting where the low type is 
bidding truthfully, whereas the high type is using
some no-regret learning algorithm. 


Let us first provide the definition of a ``mean-based'' 
no-regret learning algorithm. This was first proposed by \cite{braverman2018selling} and it has been used 
extensively in the literature (\grigorisnote{TODO: add relevant
citations.})


\grigorisnote{Another property that will probably
be useful is the following: if the cumulative utility of action $b$
is at least as large as the cumulative utility of $b'$,
then the probability of playing $b$ is at least as large
as the probability of playing $b'.$ To the best of my knowledge,
all the algorithms that have been proposed in the past have this property.}

We can show the next result under 
mean-based no-regret learning.
\begin{claim}[Last-Iterate Convergence of High-Bidder]\label{clm:last-iterate convergence of high bidder}
    Assume the the auctioneer is using second-price auction and the 
    low-valuation type is always bidding truthfully. Assume that the
    the high type is using a mean-based no-regret learning algorithm and
    let $t^* = \min \left\{t \in \nats: (t-1)\cdot(v_H - v_L) > \gamma_t \right\}$ and $\varepsilon$ be the dicretization parameter.
    Then, after
    $T$ rounds the expected revenue of the auctioneer
     is at least
    \[
        \E[\rev] \geq T\cdot v_L - \left(t^\star - \frac{v_L}{\varepsilon} \cdot \sum_{t = t^\star}^T \gamma_t\right) \,.
    \]
\end{claim}

\begin{proof}
The proof is not very hard and it follows,
essentially, by the definition of mean-based
no-regret learning and a union bound over the actions in the interval $[0,v_L].$
\end{proof}

\subsection{High Valuation Bidder is Truthful}\label{sec:high valuation truthful, low valuation learner}


\begin{claim}[Second Price Auction Revenue]\label{clm:second price auction revenue in setting with one truthful, one learner}
    For any distribution $F$ of the bidders, 
    if the low valuation agent is using the multiplicative 
    weights update (MWU) algorithm\grigorisnote{TODO: add more general
    algorithms, this also holds for $\eps$-greedy and, in general, any ``symmetric'' algorithm} the expected revenue of the auctioneer
    under the second-price auction is $v_L/2.$
\end{claim}

\begin{proof}[Proof Sketch]
    The proof is even simpler than \cite{kolumbus2022auctions}. 
    The low valuation bidder gets no signal at all as they never
    win the auction, so they keep bidding uniformly
    at random among the actions they have, i.e.,
    the interval $[0,v_L]$. Hence, they bid $v_L/2$ on average
    and this is the revenue of the auctioneer.
\end{proof}

\begin{claim}[$\rtruth(\alpha)$ Revenue]\label{clm:rtruth revenue in single learner setting}
    Assume that $v_L, v_H$ are drawn i.i.d. from $U[1/2,1].$
    Then, $\rtruth(2)$ achieves revenue at least
    $v_L/(2\ln2)$.
\end{claim}
\grigorisnote{This is to juxtapose it with the single-shot setting where the second-price auction is optimal
among the auctions that always allocated the item (assuming the distributions are regular). We can get a better bound and for 
more general distributions, this is an example 
to show the separation. We can use the fact
that the ratio of the max over min of two i.i.d. 
uniform r.v.'s has pdf $f(z) = \frac{1}{z^2}$\footnote{See, e.g., \href{https://math.stackexchange.com/questions/662601/if-x-and-y-are-uniformly-distributed-on-0-1-what-is-the-distribution-of/662630\#662630}{here}.}
and find the optimal way to set the randomness.}

\begin{claim}[Revenue of Soft-Max Auction Under MWU]\label{clm:bad revenue of softmax under MWU}
    Assume that the high type agent is truthful and
    the low type is using MWU.
    Then, $\forall T \in \nats, \forall \varepsilon > 0,
    \exists \lambda_{T,\varepsilon} > 0$, such that, $\forall \lambda >
    \lambda_{T,\varepsilon}$ the expected revenue of the soft-max
    auction with parameter $\lambda$ satisfies
    \[
        \frac{E[\rev]}{T} \leq \frac{v_L}{2\cdot T} - \varepsilon \,.
    \]
\end{claim}

\begin{proof}
    The idea is to show that, by taking the ratio of the probabilities
    of playing any two bids, for all of them it will be very close to
    $1$. To establish that, it suffices to just consider $b = 0, b' = v_L.$
\end{proof}

The above result shows that, even though asymptotically picking
a very large $\lambda$ is the optimal choice for the learner, for 
any finite time horizon $T$, if $\lambda$ is chosen above some threshold 
and the auction is repeated only for $T$ rounds, then the (expected)
average revenue
will be half of the single-shot second-price auction.

\grigorisnote{QUESTION: Is it true that under some ``natural'' class
of auctions this is the worst possible revenue the auctioneer can get?}


\subsection{Performance of Myerson's Auction}\label{sec:revenue of Myerson's auction in the repeated auctions setting}

In this section we show that Myerson's auction achieves revenue 
at least $\mathrm{OPT}/2$. The proof contains two parts. First, we upper bound $\mathrm{OPT}$ by $T\cdot \mathrm{RevMyerson}.$ This is done in the following way.
We imagine the two valuations drawn from a correlated distribution and then submitted to the mechanism in a truthful manner.
We use the result from \cite{dobzinski2011optimal} which states that the optimal
auction for two correlated bidders can be implemented as a distribution over
deterministic truthful auctions. Importantly, these auctions have the property
that if the low type increases its bid then the revenue of the auctioneer
also increases\footnote{There are auctions in which the revenue could decrease.}
Then, we can use the fact that this correlated distribution is stochastically
dominated by the product distribution, and finally the fact that
the revenue optimal auction for the product distribution is Myerson's auction.
The lower bound follows more easily.








\grigorisnote{TODO list:
\begin{itemize}
    \item Make formal the last-iterate
    convergence arguments for 
    mean-based no-regret learners.
    
    \item In the one-truthful, one-learner
    setting find the optimal parameter for 
    various randomized auctions under uniform
    distribution.
    
    \item Find natural classes of
    distributions for which \Cref{clm:bad revenue of softmax under MWU} is a lower bound.
    
    \item Find a way to parametrize
    the auction class in \Cref{thm:symmetric optimal auction when valuations are known}.
    
    \item Show the trade-off in choosing
    the right randomness parameter $\alpha$
    of some meaningful auction class
    when the learner is the low type and 
    the truthful bidder is the high type.
    
    \item When both bidders are learners,
    explore the setting where the high type
    is eps-greedy and the low type is MWU.  
    
    \item Prove that the parameter $\lambda$ of the 
    soft-max auction is increasing in $T.$
    
    \item Prove that the optimal auction has the following
    property: if the low bidder increases their bid, then
    the revenue increases. There are truthful auctions that 
    do not satisfy the property, so revenue optimality
    must be used. 
    
    \item Prove that the optimal determistic auction
    uses a different reserve that what Myerson suggests.
\end{itemize}

}




==> rtruth.tex <==
\section{Equilibria of $\rtruth(\alpha)$ Auction}\label{sec:rtruth}
Before shifting our attention to the repeated auction setting, 
we first study the equilibria of the $\rtruth(\alpha)$
auction in the static setting. To be more precise, we consider the
problem where
two bidders with private valuations $v_H, v_L$, where $v_H > v_L$,
participate in $\rtruth(\alpha)$, for some $\alpha < v_H/v_L.$
Our first main result is to
show that there is a \emph{unique} coarse correlated equilibrium (CCE)
in this setting under which both bidders are truthful.
Let us first recall the notion of a CCE.
\begin{definition}[Coarse Correlated Equilibrium (CCE)]\label{def:coarse correlated equilibrium}
Consider a $n$-player game where the strategy space
of the $i$-th player is $\calA_i$, and their
utility function is $u_i(a_1,\ldots,a_n) \in [0,1]$
for every action profile $(a_1,\ldots,a_n) \in \calA_1 \times \ldots \times \calA_n.$
A coarse correlated equilibrium (CCE) is a probability
distribution $\calD$ over $\calA_1 \times \ldots \times \calA_n $ with the property that
\[
    \E_{(a_1,\ldots,a_n) \sim \calD}[u_i(a_1,\ldots,a_n)] \geq \E_{(a_1,\ldots,a_n) \sim \calD}[u_i(a_1,\ldots,a_i', \ldots, a_n)], \forall i \in [n], \forall a_i' \in \calA_i \,.
\]
\end{definition}
In words, a CCE is a distribution over the joint 
action space of all agents with the property that, 
if everyone commits to following the action chosen
by this distribution \emph{before observing the recommendation}, then, in expectation over the 
random draw of the actions, their utility is at least
as good as if they were playing any fixed action.
\grigorisnote{TODO:introduce Nash equilibria and correlated equilibria.} We remind the reader that the set of Nash 
equilibria of a game is contained in the set of
correlated equilibria, which is contained in the 
set of coarse correlated equilibria.

We start with the following claim that will be useful in 
our proofs.\grigorisnote{TODO: we can specify a general class
of algorithms based on a function $g(b_1,b_2) = g(b_1/b_2)$
with the properties that: i) $g(b_1/b_2) + g(b_2/b_1) = 1$, 
ii) $g(b_1/b_2) = 0$ if $b_1/b_2 \leq 1/\alpha$, $g(b_1/b_2)$ 
is strictly concave for $b_1/b_2 \in [1/\alpha, \alpha]$ 
wrt to one argument assuming the other is fixed,
iii) $g(b_1/b_2) = 1 $ if $b_1/b_2 > \alpha.$ Then show that
the function used in \cite{liaw2022efficiency} satisfies
these properties.
}
\begin{claim}\label{clm:concavity of utility function in rTruth}
    For any $\alpha > 1, v > 0, b' > 0$, the utility $u(b; v, b')$
    of a bidder who participates in $\rtruth(\alpha)$ 
    is continuous in $[0,1]$ as a function
    of $b$. Moreover: 
    \begin{itemize}
        \item If $v \leq b'/\alpha$ then the set of optimal bids
        is 
        $b^\star \in [0,v]$ and give $u(b^\star;v,b') = 0.$
        \item If $v \in (b'/\alpha, \alpha \cdot b')$ 
    then $u(b; v, b')$ is strictly increasing
    for $b \in (b'/\alpha, v)$, strictly decreasing for 
    $b \in (v, \alpha\cdot b')$, and
    the
    unique optimizer is $b^\star = v.$
    \item If $v \geq \alpha \cdot b'$, then $u(b;v,b')$ 
    is strictly increasing for $b \in (b'/\alpha, \alpha\cdot b')$ and the set of 
    optimal bids is
    $b^\star \in [\alpha \cdot b', 1]$.
    \end{itemize} 
\end{claim}
\begin{proof}
Let us recall the utility 
of a bidder with valuation $v$ who is participating
in $\rtruth(\alpha)$ when their opponent 
bids $b'$, as function of their own bid $b.$ We have that
\begin{align*}
  u(b; v, b') =
  \begin{cases}
    0, & \text{ if } b < b'/\alpha \\
    v \cdot \frac{1}{2}\cdot \left(1 + \frac{\ln (b/b')}{\ln \alpha} \right) - b' \cdot \frac{b/b' - 1/\alpha}{2\ln \alpha}, &\text{ if } b'/\alpha \leq  b < \alpha \cdot b' \\
    v - b' \cdot \frac{\alpha-1/\alpha}{2\ln \alpha}, & 
    \text{ if } b \geq \alpha \cdot b' 
    \end{cases}  \,.
\end{align*}
    Consider the derivative of $u(b; v, b')$ with respect to $b$
    in the interval $b \in [b'/\alpha, \alpha \cdot b].$ We have
    that 
    \[
        \frac{\partial u(b; v, b')}{\partial b} = 
        \frac{v}{2b\ln \alpha } - \frac{1}{2\ln\alpha} \,.
    \]
    % Similarly, for the second derivative we have that
    % \[
    %     \frac{\partial^2 u(b; v, b')}{\partial b^2} = 
    %     -\frac{v}{4 b^2\ln \alpha} < 0 \,,
    % \]
    % so we can see that the function is indeed strictly
    % concave in this interval. 
    % By setting its (first) derivative
    % equal to zero, we see that indeed $b = v$ is the unique
    % maximizer of the utility function, assuming that $v \in (b'/\alpha, \alpha \cdot b').$ 
    Notice that for $b < v, b > v$ the derivative is positive,
    negative, respectively. Thus, if $v \leq b'/\alpha$ the set 
    of optimal bids is $[0,v]$ and they all give zero utility.
    Similarly, if $v \in (b'/\alpha,\alpha \cdot b')$ then
    the utility is strictly increasing in $(b'/\alpha,v)$, strictly decreasing
    in $(v,\alpha \cdot b')$, and the unique optimizer is $b^\star = v.$
    Finally, observe that if $v > \alpha \cdot b'$, then the 
    utility function is strictly increasing in $(b'/\alpha,\alpha \cdot b')$,
    and the set of optimal bids is $b^\star \in [\alpha \cdot b',1].$
\end{proof}


\begin{theorem}[CCE of $\rtruth(\alpha)$]\label{thm:cce of rtruth}
    Consider two bidders with private valuations $v_H, v_L$
    who compete in $\rtruth(\alpha)$ for a single 
    indivisible good, where $v_L \leq v_H, v_H/v_L < \alpha.$ 
    Assume that the
    strategy sets of  bidder are the rational numbers in $[0,v_H],[0,v_L]$, respectively. 
    Then, the game
    has a unique CCE under which both bidders
    are always truthful.
\end{theorem}

\begin{proof}
We provide the proof for the case where the set of possible
bids are restricted to be rational numbers. In the case
where the bids are allowed to be continuous, the CCE
of the game is still unique, up to sets of measure zero.
Let us fix the parameter of the auction $\alpha > 1$, the valuations
of the bidders $v_L, v_H$, where 
$v_L \leq v_H < \alpha v_L$. We will refer to
the bidder with valuation $v_L, v_H$, as the 
low, high bidder, respectively.
We will make use of the observation that since that
allocation rule of $\rtruth(\alpha)$ is monotone 
and the payment rule follows Myerson's identity , bidding truthfully is a \emph{weakly} dominant
strategy, i.e., $u(v; v, b') \geq u(b; v, b'), \forall v,b,b' \in [0,1].$ \grigorisnote{TODO:
add citation}
Let $\calD$ be joint distribution over 
$\left\{[0,v_L] \cap \rats \right\} \times \left\{[0,v_H] \cap \rats \right\}.$ We denote by $\calD(b_L, b_H)$
the mass that it puts on $(b_L, b_H).$
We will show that $\calD$ is a CCE if and only if 
$\calD(v_L, v_H) = 1.$ It is not hard to see that this distribution
is indeed a CCE, since bidding $v_L, v_H$,
is a weakly dominant strategy
for the low, high player, respectively. 
We proceed with the other direction now. Assume towards 
contradiction that $\calD(b_L, b_H) = \varepsilon > 0$,
where $b_L \neq v_L$ or $b_H \neq v_H.$ Let us 
first consider the case where $b_L < v_L.$
Observe that it must necessarily be that $b_H \geq \min\{v_H, \alpha b_L\} \geq b_L$, otherwise
always playing $v_H$ instead of following the 
recommendation of the distribution is a strictly better deviation for the
high player. This is because
\begin{align}\label{eq:dominance analysis}
    \E_{(b_1,b_2) \sim \calD}[u(b_2;v_H,b_1)] &= 
    \E_{(b_1,b_2) \sim \calD}[u(b_2;v_H,b_1)| (b_1,b_2) \neq (b_L, b_H)] \cdot \Pr_{(b_1, b_2) \sim \calD}[(b_1,b_2) \neq (b_L,b_H)]  \\\nonumber +
    &u(b_H;v_H,b_L)\cdot \Pr_{(b_1, b_2) \sim \calD}[(b_1,b_2) = (b_L,b_H)] \\\nonumber
    & = \E_{(b_1,b_2) \sim \calD}[u(b_2;v_H,b_1)| (b_1,b_2) \neq (b_L, b_H)] \cdot (1-\varepsilon) + 
    u(b_H;v_H,b_L)\cdot  \varepsilon \\\nonumber
     & < \E_{(b_1,b_2) \sim \calD}[u(b_2;v_H,b_1)| (b_1,b_2) \neq (b_L, b_H)] \cdot (1-\varepsilon) + 
    u(\min\{v_H, \alpha \cdot b_L\};v_H,b_L)\cdot  \varepsilon \\\nonumber
    & \leq
    \E_{(b_1,b_2) \sim \calD}[u(v_H;v_H,b_1)| (b_1,b_2) \neq (b_L, b_H)] \cdot (1-\varepsilon) + 
    u(v_H;v_H,b_L)\cdot  \varepsilon \\\nonumber
    &= \E_{(b_1,b_2) \sim \calD}[u(v_H;v_H,b_1)] \,,\nonumber
\end{align}
where the first equality follows from the law
of total expectation, the second equality
by the definition of $\Pr_{(b_1, b_2) \sim \calD}[(b_1,b_2) = (b_L,b_H)]$,
the first inequality follows because
$\min\{v_H, \alpha \cdot b_L\}$ yields higher utility
that any $b_H < \min\{v_H, \alpha \cdot b_L\}$ (due to \Cref{clm:concavity of utility function in rTruth}), the
second inequality because
$v_H$ weakly dominates all the bids, and 
the last equality follows be definition.
So far we have shown that
$b_H \in [\min\{v_H, \alpha\cdot b_L\}, v_H].$
Notice that since $b_H \leq v_H$ and $v_L > v_H/\alpha $
it must be the case that $v_L > b_H/\alpha.$
Thus, it is not hard to see that $b_L > b_H/\alpha$,
otherwise switching to bidding $v_L$ is a strictly
better strategy for the low player, by 
a similar argument as the one we presented above. Thus, by 
\Cref{clm:concavity of utility function in rTruth} we see
that the utility function of the low player has a unique optimizer
in $v_L$ under the bid $b_H$ of the high player, 
so deviating to $v_L$ if $b_L \neq v_L$ is
a strictly better strategy for the low player.
Let us now consider the case where $b_H < v_H.$
Notice that in the previous analysis we did not
make any assumptions on $b_H$, so we can assume without
loss of generality that $b_L = v_L.$ Hence,
since $b_H < v_H < \alpha \cdot v_L = b_L$
it must be the case that $b_H < \alpha \cdot b_L.$
Thus, since $b_H < v_H, b_H < \alpha \cdot b_L $
we have that $b_H < \min\{v_H, \alpha \cdot b_L\}.$
Thus, by \Cref{clm:concavity of utility function in rTruth}
we see that switching to
$\min\left\{v_H, \alpha\cdot b_L \right\} = v_H$
yields strictly better utility for the high bidder 
in this case. 
Assume that $b_H = \alpha\cdot b_L < v_H.$ This can only happen
if $b_L < v_L.$ But in this case, switching from $b_L$ to $v_L$
is a strictly better move for the low player, and
by an analysis similar to \Cref{eq:dominance analysis}
we can see that deviating to $v_H$ yields strictly
higher utility for the high player, so 
it must be the case that $b_H = v_H.$
% Let 
% \[
% \widehat{b}_L \coloneqq \inf \left\{ b \in [0,v_L] \cap \rats :\calD_L(b) = 0 \ \right\}\,.
% \]
% Assume that $\calD_L, \calD_H$ form a Nash equilibrium.
% We claim that
% \[
%     \widehat{b}_H \coloneqq \inf \left\{ b \in [0,v_H] \cap \rats :\calD_H(b) > 0 \ \right\} \geq \min\left\{\alpha \cdot \widehat{b}_L, v_H \right\} \,.
% \]
%   It is not hard to see that $\widehat{b}_H \geq \widehat{b}_L/\alpha$. If
%   not, by definition of $\widehat{b}_H, \widehat{b}_L$ there is 
%   a bid $b$ of the high player with $\calD_H(b) > 0, b < \widehat{b}_L/\alpha$,
%  thus for every bid $b'$ of the low player we have that the high player
%  always loses the auction
%  when they bid $b$, so moving the mass from $b$ to $v_H$ is a 
%  strictly better move. Assume towards contradiction that
%  $\widehat{b}_H < \min\left\{\alpha \cdot \widehat{b}_L, v_H \right\}.$

 
% Then, by definition 
\end{proof}

Let us briefly comment on the restrictions we impose on the auction. 
Regarding the no-overbidding assumption, this is standard in the
auctions literature and it is necessary to rule out some pathological 
equilibria where the player with the lowest valuation is
always winning the auction. If we allow for continuous
bids instead of countable, then there are infinitely many
equilibria, but they are also the same with the desired
one up to a set of measure zero.

Equipped with \Cref{thm:cce of rtruth}, we can prove
a strong convergence result about no-regret
learning dynamics in such auctions. Let us
first recall a folklore result which was first shown
in the pioneering work of \cite{hart2000simple} regarding the convergence
of the time-average strategies of no-regret learning algorithms
to coarse-correlated equilibria.

\begin{theorem}[No-Regret Learning and CCEs
\cite{hart2000simple}]\label{thm:convergence 
of no-regret learning dynamics to CCEs}
Let $\calG$ be a $n$-player finite-action game and
let each player 
use a (potentially different) no-regret learning
algorithm $\calA_i, i \in \nats.$ Let $p_i^t$ be the distribution over actions
of player $i \in [n]$ in round $t$ of the game, and 
$\bar{p}_i^t = 1/t \sum_{\tau=1}^t p_i^\tau.$ Let also
$\sigma_t = \prod_{i=1}^n \bar{p}_i^t$. Then, 
for any $\varepsilon > 0$ there exists some $T \in \nats$
so that
$\sigma_T$ is an $\varepsilon$-approximate CCE of the game.

\end{theorem}


\begin{corollary}[Convergence of No-Regret Learning
Algorithms in $\rtruth(\alpha)$]\label{cor:convergence
of no-regret in rtruth}
    Assume that two bidders with private valuations
    $v_L, v_H, v_L \leq v_H$,
    participate in $\rtruth(\alpha)$, where $\alpha > v_H/v_L.$ 
    Then, for any $\varepsilon > 0$ there exists
    some $T \in \nats$ so that the average distribution 
    over bids of each player converges to a Nash
    equilibrium. \grigorisnote{TODO: write it 
    more formally}
\end{corollary}

\begin{proof}
The proof follows easily from \Cref{thm:cce of rtruth} and
\Cref{thm:convergence 
of no-regret learning dynamics to CCEs}.
\end{proof}



\grigorisnote{All the results from here on are written
informally and the proofs are just sketches.}


\begin{theorem}[Last Iterate Convergence of Mean-Based Learners]\label{thm:rtruth last iterate convergence}
Assume that both learners are using mean-based no-regret
learning algorithms and $v_H/v_L < \alpha.$ Then, the
learners convergence to truthful bidding in a last iterate manner.
\end{theorem}

\begin{proof}[Proof Sketch]
    We need to partition the time horizon into
    multiple intervals and argue that the mean-based
    property leads to repeated action elimination.
    Even though it is not a conceptually difficult
    proof, it is a bit challenging technically.
\end{proof}

\begin{claim}[Choice of $\alpha$]\label{clm:optimal choice of alpha
for fixed valuation}
    Let two bidders with private valuations
    $v_L, v_H, v_L < v_H$, bid truthfully in
    $\rtruth(\alpha).$ Let $\beta = v_H/v_L$.
    Then, the revenue
    of the auctioneer is
    \begin{align*}
        \rev(\alpha) = 
        \begin{cases}
        \frac{v_L}{2} \cdot \frac{\alpha - 1/\alpha}{\ln \alpha}, & \text{ if } 1 < \alpha \leq \beta \\
        \frac{v_L(\beta+1)}{2} \cdot \left(\frac{\alpha-1}{\alpha \ln \alpha} \right), & \text{ if } \alpha > \beta
        \end{cases}
        \,.
    \end{align*}
    and it holds that
    \[
        \sup_{\alpha > 1} \rev(\alpha) = \frac{v_L(\beta^2 - 1)}{2\beta \ln 
        \beta} \,.
    \]
\end{claim}

\begin{proof}
    Let us first consider the revenue of auction
    when $\alpha \leq \beta.$
    By definition of the allocation rule, the 
    high bidder always wins the auction and the payment is
    $v_L\cdot(\alpha - 1/\alpha)/(2\ln \alpha).$
    Let $g(\alpha) = \frac{\alpha-1/\alpha}{\ln \alpha}.$
    Then 
    \[
        g'(\alpha) = \frac{a^2 \ln \alpha + \ln\alpha + 1 -\alpha^2}{(\alpha \ln\alpha)^2} \,.
    \]
    Notice that $g'(1) = 0.$ Moreover,
    \[
        \frac{d}{d\alpha} \left(a^2 \ln \alpha + \ln\alpha + 1 -\alpha^2  \right) = 2\alpha \ln \alpha + \frac{1}{\alpha} - \alpha > 0, \forall \alpha > 1 \,.
    \]
    Thus, $\rev(\alpha)$ is increasing in the interval $\alpha \in (1,\beta).$
    Let us consider the case where $\alpha > \beta.$ Notice 
    that the revenue is continuous.
    We have that
    \begin{align*}
        \rev(\alpha) &= 
           v_L \cdot \frac{v_H/v_L - 1/\alpha}{2\ln \alpha} + 
           v_H \cdot \frac{v_L/v_H - 1/\alpha}{2\ln \alpha} \\
           &= 
           v_L \cdot \frac{v_H/v_L - 1/\alpha}{2\ln \alpha} + 
           v_L \cdot \frac{1 - v_H/(v_L\cdot\alpha)}{2\ln \alpha}\\
           &= 
           \frac{v_L}{2}\cdot
           \left( \frac{\beta + 1 - \frac{\beta+1}{\alpha}}{\ln\alpha} \right) & & \beta = v_H/v_L \\
           &=  \frac{v_L  (\beta + 1)}{2} \cdot
           \left(\frac{\alpha - 1}{\alpha  \ln \alpha}\right) \,.
    \end{align*}
    Let us define $f(\alpha) = \frac{\alpha-1}{\alpha \ln \alpha}.$
    Then, its derivative is $f'(\alpha) = \frac{\alpha\ln \alpha - (\alpha - 1)(\ln \alpha + 1)}{(\alpha \ln \alpha)^2} = \frac{\ln \alpha - \alpha + 1}{(\alpha \ln \alpha)^2} < 0, \forall \alpha > 1.$ 
    Thus, we can see that the optimal choice is $\alpha = \beta$, i.e.,
    \[
        \sup_{\alpha > 1} \rev(\alpha) = \rev(\beta) = 
        \frac{v_L(\beta^2 - 1)}{2\beta \ln 
        \beta} \,.
    \]
\end{proof}


\begin{claim}[Revenue Maximizing Auction for i.i.d. Bidders]
    Let two bidders with valuations $v_1, v_2$ drawn i.i.d.
    from a regular distribution $F$ participate in some auction. 
    Then, among all the auctions that always allocate the item 
    the second-price auction maximizes the revenue of the auctioneer.
\end{claim}

\begin{proof}
    The proof follows from Myerson's lemma.
\end{proof}


We focus on the following interaction between the auctioneer
and two bidders who are using a no-regret learning algorithm
to bid in the auction repeatedly. We assume that their valuation
is drawn i.i.d. from some known regular distribution $F$
at the beginning of the interaction.
\begin{itemize}
    \item The auctioneer sets the parameter $\alpha$ of
    the auction $\rtruth(\alpha)$ knowing the valuation distribution
    $F$ of the bidders.
    \item The values $v_1, v_2 \sim F$ are realized.
    \item The bidders participate in the auction repeatedly using
    a no-regret learning algorithm.
\end{itemize}

\grigorisnote{I am not sure how to prove that claim. 
It looks like it requires us to understand
the asymptotic distribution of the second-price
auction first, and we don't seem to have a
handle on it.}

\begin{claim}[$\rtruth(\alpha)$ Outperforms Second-Price]\label{clm:
rtruth outperforms second price}
    There exists a distribution $F$, no-regret learning algorithms,
    and a parameter $\alpha$
    such that the revenue of the auctioneer under $\rtruth(\alpha)$
    is strictly larger than the revenue under the second-price auction
    as $T \rightarrow \infty.$
\end{claim}

\begin{proof}[Proof Sketch]
\grigorisnote{This is not correct yet. We can play around with the idea that the high guy uses eps-greedy and the low guy uses MWU.}
    Let $F = U[1-\varepsilon, 1]$ for some $\varepsilon > 0$ that is 
    sufficiently small. Let $\alpha = \frac{1}{1-\eps}.$
    Assume without loss of generality that $v_1 \geq v_2.$
    Notice that under this choice of $\alpha$ we have that
    $v_1/v_2 < \alpha$, so by \Cref{cor:convergence
of no-regret in rtruth} we have that as $T \rightarrow \infty$
the bid distribution of both bidders converges to truthful bidding. 
Let $\beta = v_1/v_2.$ From \Cref{clm:optimal choice of alpha
for fixed valuation} we know that the revenue of $\rtruth(\beta)$ is
strictly larger than the revenue of the second price auction.
Moreover, we have that $\beta < \alpha < \beta + O(\varepsilon)$, so
by continuity of the revenue function we have that $\rev(\rtruth(\alpha)) > 
\rev(\rtruth(\beta)) - O(\varepsilon) > \rev(\spr) - O(\varepsilon).$
Thus, we can see that for large enough $T$, the average
revenue of every auction is at most $\varepsilon$ less than the revenue of 
the second price auction. More formally,
for any constant $c > 0$ there is some 
small enough $\varepsilon > 0$ so
that 
\[
    \frac{1}{1-\eps} < 1 + (1+c)\eps \,.
\]
Moreover, when $\alpha > \beta > 1$, we have that
the derivative of the revenue function
with respect to $\alpha$ is
\[
   \frac{ v_L(\beta + 1)}{2}\cdot
   \frac{1-\alpha+\ln \alpha}{(\alpha \ln \alpha)^2} \,.
\]
Thus for $\alpha > 1$, the Lipschitz constant is at most
\[
    \left\lvert \frac{ v_L(\beta + 1)}{2}\cdot
   \frac{1-\alpha+\ln \alpha}{(\alpha \ln \alpha)^2} \right\rvert \leq \frac{v_L(\beta+1)}{4} \,.
\]
Moreover, since $\beta < 1/(1-\eps)$ we can
further bound this quantity as
\[
    \frac{v_L\left(2+(1+c)\cdot\eps\right)}{4} < \frac{2+(1+c)\cdot\eps}{4}\,.
\]
By picking $\alpha = 1/(1-\eps)$ we have
that $0 < \alpha - \beta < (1+c)\eps$.
Hence, the revenue of our auction is
worse than the revenue of the second price
auction by an additive
\[
    \frac{2+(1+c)\eps}{4}\cdot(1+c)\eps < \frac{2(1+c')\eps}{4} \,.
\]
\grigorisnote{More formally, for any $c'$
we can pick an $\eps$ so that the above holds.}
Adding the convergence error, we see that
the revenue is worse by an additive
\[
    \frac{2(1+c')\eps}{4} + \eps' \,,
\]
compared to the second price, where $\eps' \rightarrow 0$ as $T \rightarrow \infty.$


Let us now focus on the long-term revenue of the second price auction
in this setting. \grigorisnote{Still working on it.}
\end{proof}



This can lead to various corollaries regarding 
equilibria of various auctions we consider in this paper. Compare
to the results of \cite{kolumbus2022auctions, kolumbus2022and} which show that 
for second-price auctions, this meta-game
has bad equilibria and can be 
manipulated.



==> softmax.tex <==
\section{Randomized Auction Using Soft-Max}\label{sec:mwu auction}
In this section we consider a randomized auction that is based on the
soft-max selection rule. To the best of our knowledge, this allocation
rule in the context of mechanism design was first proposed in \cite{mcsherry2007mechanism}. This auction
is parametrized by a number $\lambda > 0$ so we denote it by $\softmax(\lambda).$
The allocation rule is defined as follows. Given bids $b, b'$ the probability
that bidder who submitted $b$ wins is
\[
    \Pr[b \text{ wins }|b'] = \frac{e^{\lambda \cdot b}}{e^{\lambda \cdot b} + e^{\lambda \cdot b'}} = \frac{1}{1 + e^{\lambda\cdot(b'-b)}} \,.
\]
It is not hard to see that this allocation rule is (strictly) increasing in $b$, 
for any $b' \in \reals.$ Thus, the payment rule that induces a truthful auction
can be computed by Myerson's formula as
\begin{align*}
     p(b|b') &= b \cdot \Pr[b \text{ wins }|b'] - \int_{0}^b \Pr[z \text{ wins }|b'] dz\\
     &= b \cdot \frac{1}{1+e^{\lambda\cdot(b'-b)}} - \frac{1}{\lambda} \ln\frac{e^{\lambda\cdot b}+ e^{\lambda\cdot b'}}{1 + e^{\lambda\cdot b'}}
\end{align*}

\begin{lemma}[Truthfulness is Strictly Dominant in Soft-Max Auctions]
\label{lem:truthfulness is strictly dominant in soft-max auctions}
For any bidder, no matter what their opponent bids, truthful
bidding is a strictly dominant strategy.
\end{lemma}

\begin{proof}
    Consider a bidder with valuation $v \geq 9$ and let $b'$ be the bid of the competing bidder. Let $u(b|b')$
    be the utility, i.e., $u(b|b') = v\cdot \Pr[b \text{ wins }|b'] - p(b|b').$ By taking the partial derivative with respect to $b$
    we see that
    \begin{align*}
        \frac{\partial u(b|b')}{\partial b} &=
        \frac{\partial\left((v-b) \Pr[b \text{ wins }|b'] + \int_{0}^b \Pr[z \text{ wins }|b'] dz \right)}{\partial b}\\
        &= (v-b)\frac{\partial \Pr[b \text{ wins }|b']}{\partial b} \\
        &= (v-b)\frac{\lambda\cdot e^{\lambda \cdot (b'-b)}}{(1+ e^{\lambda \cdot (b'-b)})^2} \,.
    \end{align*}
    Thus, for $b < v$ the function is strictly increasing whereas for
    $b > v$ the function is strictly decreasing. Hence, the unique
    optimal solution is $b^\star = v.$
\end{proof}

\begin{corollary}[Equilibria of Sigmoid Auction]\label{cor:equilibria of sigmoid}
For any $\lambda > 0, v_L, v_H \geq 0$
the only Nash equilibrium of
the sigmoid auction is truthful bidding.
\end{corollary}

\begin{proof}
    Follows immediately from the previous result.
\end{proof}

\begin{theorem}[Revenue of Sigmoid Auction]\label{thm:revenue of signoid auction}
There exists a choice of $\lambda$ such that
the revenue of the sigmoid auction can be arbitrarily close
to the revenue of the second price auction.
\end{theorem}

\begin{proof}[Proof Sketch]
    The idea is that we can approximate the allocation rule
    of the second-price auction, i.e., the step function at $b'$
    as close as we want to, hence the payments will also be 
    as close as we want them to with the second price auction.
\end{proof}

\begin{theorem}[Last Iterate Convergence]\label{thm:last iterate convergence in sigmoid auctions}
If both players are using a mean-based no-regret learning
algorithm then they convergence to bidding truthfully
in a last-iterate manner.
\end{theorem}

\begin{proof}[Proof Sketch]
    The proof is a bit more technical. The idea is that the 
    reward of the truthful action will be significantly
    better than the reward of the best so all the mass will move
    there (using the mean-based property).
\end{proof}

\begin{lemma}[Optimal Choice of $\lambda$]\label{lem:optimal choice of lambda for softmax auction}
The revenue optimal choice of the
randomness parameter is $\lambda = ??$
and the revenue of the auctioneer is $??.$
\end{lemma}

\begin{proof}
\grigorisnote{It is not clear how to characterize
the optimal revenue of this auction. In some cases,
we need to take $\lambda \rightarrow \infty$ and
in some other cases the optimal revenue is 
achieved by picking some finite $\lambda.$ It 
is very messy to understand what's the case
and I don't think it adds much value. We can
leave as a comment that sometimes the revenue optimal
auction generates more revenue than the second price
auction and sometimes it generates the same revenue 
(even when the valuation are known to the auctioneer).}
    By the definition of the payment rule
    of this auction, assuming 
    truthful bidding of the bidders,
    we have for any $\lambda > 0$ that
    \[
        \rev(v_L,v_H,\lambda) = 
        \frac{v_H e^{\lambda \cdot v_H} + v_L e^{\lambda \cdot v_L}}{e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L}} - \frac{1}{\lambda} \cdot \ln\left(\frac{(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L})^2}{(1+e^{\lambda \cdot v_L})\cdot(1+e^{\lambda \cdot v_H})}\right) \,,
    \]
    whereas $\rev(v_L,v_H,0) = 0.$
    
    Let us first consider $\lim_{\lambda \rightarrow \infty} \rev(v_L,v_H,\lambda).$
    We calculate each term of the limit separately.
    For the first term, we have that
    \begin{align*}
        \lim_{\lambda \rightarrow \infty} \frac{v_H e^{\lambda v_H} + v_Le^{\lambda v_L}}{ e^{\lambda v_H} + e^{\lambda v_L}} &= 
         \lim_{\lambda \rightarrow \infty} \left( v_H \frac{e^{\lambda v_H}}{e^{\lambda v_H} + e^{\lambda v_L}} + v_L \frac{e^{\lambda v_L}}{e^{\lambda v_H} + e^{\lambda v_L}}\right)\\
         &=  \lim_{\lambda \rightarrow \infty} \left( v_H \frac{1}{1 + e^{\lambda (v_L - v_H)}} + v_L \frac{1}{1 + e^{\lambda (v_H - v_L)}}\right)\\
         &= v_H \,,
    \end{align*}
    since $v_H \geq v_L.$
    Let us now focus on the second term. Notice
    that since $\ln(x)$ is continuous we have that $\lim_{\lambda \rightarrow \infty} \ln(f(\lambda)) = 
    \ln(\lim_{\lambda \rightarrow \infty}) f(\lambda)$ if
    $\lim_{\lambda \rightarrow \infty} f(\lambda)$
    exists and is positive. We have that
    \begin{align*}
        \lim_{\lambda \rightarrow \infty} \ln\left(\frac{(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L})^2}{(1+e^{\lambda \cdot v_L})\cdot(1+e^{\lambda \cdot v_H})}\right) &= \lim_{\lambda \rightarrow \infty} \ln \left( \frac{(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L})\cdot(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L}) }{(1+e^{\lambda \cdot v_L})\cdot(1+e^{\lambda \cdot v_H})} \right) \\
        &= \lim_{\lambda \rightarrow \infty}\ln \left( \frac{e^{\lambda v_L}}{1+e^{\lambda v_L}} \cdot \frac{e^{\lambda v_H}}{1+e^{\lambda v_H}} \cdot (1+e^{\lambda(v_H - v_L)}) \cdot (1 + e^{\lambda(v_L - v_H)}\right) \\
        &= \lim_{\lambda \rightarrow \infty} \left( \ln \frac{e^{\lambda v_L}}{1+e^{\lambda v_L}} + \ln \frac{e^{\lambda v_H}}{1+e^{\lambda v_H}} + \ln\left( 2 + e^{\lambda(v_H - v_L)} + e^{\lambda(v_L - v_H)} \right)\right) \,.
        % &= \lim_{\lambda \rightarrow \infty} \ln\left( 2 + e^{\lambda(v_H - v_L)} + e^{\lambda(v_L - v_H)} \right) \,.
    \end{align*}
    Thus,
    \begin{align*}
        \lim_{\lambda \rightarrow \infty} \frac{\ln\left(\frac{(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L})^2}{(1+e^{\lambda \cdot v_L})\cdot(1+e^{\lambda \cdot v_H})}\right)}{\lambda } &= \lim_{\lambda \rightarrow \infty} \frac{\ln \frac{e^{\lambda v_L}}{1+e^{\lambda v_L}} + \ln \frac{e^{\lambda v_H}}{1+e^{\lambda v_H}} + \ln\left( 2 + e^{\lambda(v_H - v_L)} + e^{\lambda(v_L - v_H) } \right)}{\lambda} \\
        &= \lim_{\lambda \rightarrow \infty}
        \frac{\ln\left( 2 + e^{\lambda(v_H - v_L)} + e^{\lambda(v_L - v_H) } \right)}{\lambda} \\
        &= v_H - v_L \,.
    \end{align*} 
    Putting it together, we see that
    \[
        \lim_{\lambda \rightarrow \infty} \rev(v_L, v_H, \lambda) = v_H - (v_H - v_L) = v_L \,.
    \]
    In order to prove the result, it suffices
    to show that $\rev(v_L,v_H,\lambda)$
    is increasing in $\lambda.$ We consider
    each term separately. For the first term,
    we have that
    \begin{align*}
        \frac{\partial\left( \frac{v_H e^{\lambda \cdot v_H} + v_L e^{\lambda \cdot v_L}}{e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L}}\right)}{\partial \lambda} &= \frac{(v_H - v_L)^2 e^{\lambda(v_L + v_H)}}{\left( e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L}\right)^2} \geq 0 \,,
    \end{align*}
    and the equality holds if and only if 
    $v_H = v_L$, in which case the revenue is
    always constant and equal to $v_L = v_H.$ 
    Thus, the first term is indeed increasing in $\lambda$. 
    Let us now focus on the second term and
    let 
    \[
        f(\lambda) =  \ln\left(\frac{(e^{\lambda \cdot v_H} + e^{\lambda \cdot v_L})^2}{(1+e^{\lambda \cdot v_L})\cdot(1+e^{\lambda \cdot v_H})}\right) \,.
    \]
    In order to show that $f(\lambda)/\lambda$ is decreasing
    it suffices to show that $f$ is increasing and 
    it is concave. Indeed assume that this is the case
    and consider $\lambda_1 < \lambda_2.$ Notice that
    $f(0) = 0$ and since $f$ is increasing, $f(\lambda) > 0$
    for all $\lambda > 0.$
    Then we need
    to show that
    \begin{align*}
        \frac{f(\lambda_2)}{\lambda_2} &< \frac{f(\lambda_1)}{\lambda_1} &\iff & \quad (f(\lambda_1) > 0, \lambda_2 > 0)\\
        \frac{f(\lambda_2)}{f(\lambda_1)} &< \frac{\lambda_2}{\lambda_1} &\iff \\
        \frac{f(\lambda_1) + \int_{\lambda_1}^{\lambda_2} f'(z)dz}{f(\lambda_1)} &< \frac{\lambda_1 + (\lambda_2-\lambda_1)}{\lambda_1} &\iff  & \quad (f(0) = 0) \\
        \frac{\int_{\lambda_1}^{\lambda_2} f'(z) dz}{\int_{0}^{\lambda_1}f'(z)dz} &<  \frac{\lambda_2-\lambda_1}{\lambda_1} \,,
    \end{align*}
    where the last inequality holds since $\int_{\lambda_1}^{\lambda_2} f'(z) dz < f'(\lambda_1)\cdot (\lambda_2-\lambda_1), \int_{0}^{\lambda_1} f'(z) dz > f'(\lambda_1)\cdot \lambda_1$ due to the concavity of $f,$
    and $f'(\lambda) > 0$ for all $\lambda > 0.$
    Let us first show that $f$ is indeed increasing.
    Taking
    the partial derivative with respect to
    $\lambda$ we get\footnote{This can be 
    verified on Wolfram using the following
     \href{https://tinyurl.com/wolframSoftMaxDerivative}{link} (alternate form). }
    \begin{align*}
\frac{\partial f}{\partial \lambda} = \frac{v_L (e^{\lambda (v_L + v_H)} + e^{\lambda (2 v_L + v_H)} - e^{\lambda (v_L + 2 v_H)} + 2 e^{\lambda v_L} + e^{2 \lambda v_L}) + v_H (e^{\lambda (v_L + v_H)} - e^{\lambda (2 v_L + v_H)} + e^{\lambda (v_L + 2 v_H)} + 2 e^{\lambda v_H} + e^{2 \lambda v_H})}
{(e^{\lambda v_L} + 1) (e^{\lambda v_H} + 1) (e^{\lambda v_L} + e^{\lambda v_H})} \,.
\end{align*}
In order to show that this expression is 
non-negative it suffices to show that
\begin{align*}
    v_L\cdot\left(e^{\lambda(2v_L + v_H)} - e^{\lambda(2v_H + v_L)}\right) + v_H\cdot\left(e^{\lambda(2v_H + v_L)} - e^{\lambda(2v_L + v_H)}\right) &\geq 0 &\iff\\
    e^{\lambda(2v_H + v_L)}(v_H - v_L) - e^{\lambda(2v_L + v_H)}(v_H - v_L) & \geq 0 & \iff \\
    (v_H - v_L) \cdot \left(e^{\lambda(2v_H + v_L)} - e^{\lambda(2v_L + v_H)} \right) &\geq 0 \,,
\end{align*}
which holds since $v_H \geq v_L$ and $\lambda > 0.$ We now
focus on providing sufficient conditions 
for the concavity of $f.$
\end{proof}



